HybridPose: 6D Object Pose Estimation under Hybrid Representations

We introduce HybridPose, a novel 6D object pose estimation approach. HybridPose utilizes a hybrid intermediate representation to express different geometric information in the input image, including keypoints, edge vectors, and symmetry correspondences. Compared to a unitary representation, our hybrid representation allows pose regression to exploit more and diverse features when one type of predicted representation is inaccurate (e.g., because of occlusion). Different intermediate representations used by HybridPose can all be predicted by the same simple neural network, and outliers in predicted intermediate representations are filtered by a robust regression module. Compared to state-of-the-art pose estimation approaches, HybridPose is comparable in running time and accuracy. For example, on Occlusion Linemod dataset, our method achieves a prediction speed of 30 fps with a mean ADD(-S) accuracy of 47.5%, representing a state-of-the-art performance. The implementation of HybridPose is available at https://github.com/chensong1995/HybridPose.

==> Backup/03_overview.tex <==
\section{Overview}
\label{Section:Overview}


In an abstract form, our approach shall look like this. Consider an input domain $\set{D}_s$ and a collection of intermediate representations $\set{D} = \{\set{D}_1,\cdots, \set{D}_n\}$. Our goal is to train 3D sets of neural networks:
\begin{itemize}
\item Prediction networks $f_{\theta_i}: \set{D}_s \rightarrow \set{D}_{i}, 1\leq i \leq n$.
\item Conversion networks $f_{\theta_{ij}}:\set{D}_i \rightarrow \set{D}_j$ and some (if not all of these networks) have trainable parameters.
\item Pose estimation network $g_{\theta}: \set{D}_1\times \set{D}_2\times \cdots \times \set{D}_n \rightarrow SE(3)$ that takes the predicted representations as input and outputs a 6D pose. This network may be implemented as a reweighted least square.
\end{itemize}

Regarding training, we consider
\begin{itemize}
\item Self-supervision constraints such as
\begin{equation}
f_{\theta_{ij}}\circ f_{\theta_{i}} = f_{\theta_j}, \quad 1\leq i\neq j \leq n.    
\end{equation}
Training such networks can utilize unlabeled data.
\item Training each $f_{\theta_i}$ can utilize labeled data.
\item Training each $f_{\theta_{ij}}$ can utilize geometric constraints or data for other tasks. However, we need to make sure things are properly evaluated.
\item We may impose an end-to-end lose on the final predicted pose.
\end{itemize}

==> Backup/04_approach.tex <==
\section{Chen Song: Approach}
\label{Section:Approach}
\begin{comment}
Given a 2D RGB image, the ultimate goal of 6D pose estimation is to detect and estimate the pose of a set of known objects in the camera space. Each pose is represented by a 6-tuple $(\textit{R}; \textbf{t})$, where $\textit{R}$ is the rotation parameters and $\textbf{t}$ is the translation parameters. $(\textit{R}; \textbf{t})$ transforms the object from the origin of the camera space to its actual position.

Similar to previous works (CITATION NEEDED), our work uses a two-stage pipeline. The first stage of the pipeline predicts the 2D location of a fixed number of keypoints for each object in the image. These predicted keypoints are treated as intermediate representations of objects of interests, and the second stage of the pipeline computes the 6D pose $(\textit{R}; \textbf{t})$ according to the intermediate representations. The novelties of our work are:

\begin{itemize}
  \item We detect and use symmetric features to assist the keypoint prediction process.
  \chensong{\item We treat detected symmetric features as a second intermediate representation of objects of interests, and use keypoints and symmetric features collaboratively to compute the 6D pose.}
\end{itemize}


\subsection{Stage I: Intermediate feature prediction}
\mysubsubsection{Keypoint selection}
A set of $K$ keypoints is selected from each 3D object in the dataset. To determine the location of the $K$ keypoints, we first manually label the axis of reflection symmetry on each object. A method based on the farthest point sampling (FPS) algorithm proposed in~\cite{pvnet} is then used to select $K/2$ keypoints. These $K/2$ keypoints are mirrored with respect to the labeled axis of symmetry, and the closest points on the 3D object to the mirrored keypoints are selected as an additional $K/2$ points.

\qixing{1.Before doing that, can we make PVNET trainable end-to-end.}

\qixing{2.it seems to me we do not need powerful tools such as GAN. Simply, we want the predicted symmetric correspondence flow to be compatible with the symmetric relations among key points, and this constraint can be formulated explicitly.}

\qixing{3. That being said, we do need to consider neural networks to transfer one domain into another when incorporating additional intermediate representations.}

\mysubsubsection{CycleGAN-based intermediate feature prediction}
The success of CycleGAN~\cite{cyclegan} and DualGAN~\cite{dualgan} demonstrates the power of combining cycle consistent and adversarial loss in training domain transfer networks. RGB images, keypoints, and symmetric features can be viewed as three different domains of the same scene. Identical to~\cite{pvnet}, we represent keypoints using unit vectors and semantic labels. Inspired by~\cite{beyond-planar-symmetry}, we represent symmetric feature using a possibility heatmap of the reflection symmetry axis. Since unit vectors, semantic labels, and the heatmap are all 2D matrices, and their dimensions are the same to the initial RGB image, it is natural to formulate intermediate feature prediction as a supervised image-to-image translation problem.

Using the terminologies in Generative Adversarial Nets (GANs), we train six different generators to allow the translation among the three domains. As shown in Figure 1 (TODO), $G_{IK}$ and $G_{KI}$ translate between RGB images and keypoints. $G_{KS}$ and $G_{SK}$ translate between keypoints and symmetric features. $G_{IS}$ and $G_{SI}$ translate between 2D RGB images and symmetric features.

At inference time, only $G_{IK}$ and $G_{IS}$ are used to predict keypoints and symmetric features from the input RGB image. At training time, the rest four generators and all six discriminators are used to assist the training of $G_{IK}$ and $G_{IS}$.

\mysubsubsection{Stage II: 6D pose computation}
\end{comment}

This section introduces an end-to-end trainable network which utilizes keypoints and symmetry information.

\begin{enumerate}
    \item We use $f_{I \rightarrow K}$ to extract $N$ ($N > 4$) 2D keypoints from the input RGB image. This keypoint extraction is formulated as a regression problem from RGB images to keypoint coordinates. $f_{I \rightarrow K}$ is implemented as a neural network.
    \item We use $f_{I \rightarrow S}$ to extract the axis of reflection symmetry from the input RGB image. $f_{I \rightarrow S}$ is implemented as a second neural network as described in~\cite{beyond-planar-symmetry}.
    \item The $N$ keypoints are symmetrically selected at training time, and their coordinates extracted in step 1 are refined according to the axis of reflection symmetry obtained in step 2. This refinement increases the robustness of the proposed pose estimation network in noisy environments and under occlusions.
    \item We randomly select 4 out of all $N$ keypoints after the refinement. We require these 4 keypoints to be symmetric with respect to the axis of relection obtained in step 2. We then use Perspective-3-Point~\cite{p3p} to create a hypothesis of the 6D pose. Note that while the general Perspective-N-Point point problem is not differentiable, the special case when $N = 3$ is. We repeat this step to generate a pool of hypotheses of the 6D pose. \chensong{Correct me if I am wrong here}
    \item We use DSAC~\cite{dsac}, a differentiable variant of RANSAC, to select and refine the best hypothesis from the pool. The reprojection error used in DSAC is here only defined over $N$ keypoints.
\end{enumerate}


\section{Grem: Cycle consistency for directed graph}
\subsection{Overview}
\begin{figure}[ht]
\centering
\includegraphics[width=0.95\linewidth]{cycle.png}
\caption{Architecture}
\label{Fig: Architecture}
\end{figure}
The key idea of our method is to train different domains $\set{D}_{1:3}$, keypoint, object pose and symmetry simultaneously, by enforcing consistent constraints among network outputs along a cycle direction. We form $\set{D}_{1:3}$ as a directed graph in Fig\ref{Fig: Architecture}, and propose that by satisfying the cycle constraints among domains, the training of each domain will help with each other and get higher accuracy.

As indicated in Fig.\ref{Fig: Architecture}, our architecture has four individual networks:
\begin{itemize}
\item $f_{\theta_0}: \set{D}_s \rightarrow \set{D}_{0}$, which predicts dense  symmetric  correspondence $\set{D}_{0}$ from source RGB image $\set{D}_s$.
\item $f_{\theta_1}: \set{D}_s \rightarrow \set{D}_{1}$, named PVNet, which predicts sparse symmetric keypoints $\set{D}_1:p_i p'_i$ from input image $\set{D}_s$. 
\item $f_{\theta_{2}}: \set{D}_1 \rightarrow \set{D}_{2}$, named PnPNet, which predicts object pose $\left[R| t\right]$ denoted by $\set{D}_2$, given 3D-2D correspondence.
\item $f_{\theta_{3}}: \set{D}_0 \rightarrow \set{D}_{3}$, named symmetry voting network, which predicts symmetry plane parameters $R_s t_s$ denoted by $\set{D}_3$ from dense symmetric correspondence $\set{D}_{0}$. 
\end{itemize}

To enforce the consistency of different domains $\set{D}_{1:3} = \{\set{D}_1,\cdots, \set{D}_3\}$, we exploit the following geometric constraints:
\begin{enumerate}
    \item $f_{\theta_{1,2}}: \set{D}_1 \rightarrow \set{D}_{2}$. Essentially, $f_{\theta_{1,2}}$ is PnPNet $f_{\theta_{2}}$ , which estimates object pose by leveraging 3D-2D correspondence, and enforces the consistency of pose and keypoint implicitly. 
    \item $f_{\theta_{2,3}}:\set{D}_2 \rightarrow \set{D}_{3}$: maps object pose $\left[R| t\right]$ to symmetry plane parameters $R_s t_s$ by:
    \begin{equation}
        \begin{aligned}
        t_s &= 2t^{\mathrm{T}}R\vec{n}R\vec{n}\\
         R_s & = I - 2R\vec{n}R\vec{n}^{\mathrm{T}}
        \end{aligned}
    \end{equation}
    where $\vec{n}$ is normal vector of symmetry plane in object frame. This equation enforces the consistency of pose and symmetry and will be further discussed in section [SYMMETRY].
  
    \item $f_{\theta_{3,1}}:\set{D}_3 \rightarrow \set{D}_{1}$ enforces the consistency between symmetry plane parameters $R_s t_s$ and symmetric keypoint pairs $(p p')$ by:
    \begin{equation}
        x\in N(p'^{T}K^{-T}t_s^{\wedge}R_sK^{-1})
    \end{equation}
    where $N(M)$ denotes the null-space vector of $M$. The derivation of this equation will be discussed in Session [SYMMETRY].
\end{enumerate}

We briefly summarize our training procedure as follows:
\begin{enumerate}
    \item We first train network $f_{\theta_0}$ to predicts dense symmetry correspondences.
    \item We train network $f_{\theta_3}$ to votes symmetry plane parameters $R_s t_s$.
    \item We train sparse symmetric keypoints using PVNet $f_{\theta_1}$. 
    \item $f_{\theta_2}$ PnPNet  takes in PVNet's output and predicts pose $\left[R| t\right]$. 
    \item Given pose $\left[R| t\right]$ and constraint $f_{\theta_{2,3}}$, the symmetry voting network $f_{\theta_3}$ is retrained.
    \item Given symmetry plane parameters $R_s t_s$ and leveraging constraint $f_{\theta_{3,1}}$, the PVNet $f_{\theta_1}$ is retrained.
    \item Repeat step 4-6 until cycle consistency is satisfied.
\end{enumerate}

The loss of network $f_{\theta_1}$ and $f_{\theta_3}$ has two parts: supervised loss and cycle consistency loss. PnPNet is trained separately. 

We will discussed the network details and symmetry in the following sessions.



\subsection{Refinement Approach Overview}
Our approach is motivated by a fact that most of objects are reflection symmetric which can be exploited for better pose estimation. Therefore we propose to first implement PnP-based pose estimation with predicted keypoints and further leverage both the symmetric and keypoint features to refine the pose in a recurrent manner.

\begin{figure}
\centering
\includegraphics[width=0.95\linewidth]{arch_draft.pdf}
\caption{Architecture draft}
\label{Fig: Architecture2}
\end{figure}
As illustrated in \ref{Fig: Architecture2}, our architecture contains four parts: keypoint prediction module, symmetry prediction module, pose refinement module, and feature conversion module. 

\begin{itemize}
\item Keypoint prediction module implements the same strategy in PVNet and generates the initial object pose $T$ using EPnP method.
\item Symmetry prediction module generates pixel-wise vector pointing from the current visible 2D pixel point to its symmetric point in 2D image, which is further utilized in pose refinement module. 
\item Pose refinement network $g_{\theta}$ operates on each predicted keypoint and corresponding symmetry vector to generate the pose update $\Delta T$ recurrently. At $k$ th iteration, $g_{\theta}$ takes the input pose $T_k$, keypoint reprojection error and symmetry reprojection error and outputs the pose update $\Delta T_{k+1}=\varepsilon_{k+1}$ in $\mathfrak{se(3)}$. The new pose is then updated to $T_{k+1} = \mathrm{exp}(\varepsilon_{k+1}^{\wedge})T_k$. $T_{k+1}$ is the input in $k+1$ iteration. 

Given the predicted keypoints and symmetry vector, as well as initial pose, the network is trained end-to-end by minimizing the difference between ground truth pose and updated pose.
\item Conversion module enforces the consistency of keypoint and symmetry feature under a certain pose $T$. Conversion module is independent of pose refinement network but will change the input of pose refinement network by providing better keypoint and symmetry information.
\end{itemize}

\subsection{Keypoint}
Similar to PVNet. The network generates $n$ keypoints and we use known 3D coordinates to estimate initial pose using PnP algorithm.
\subsection{symmetry prediction module}
Assume the object has one reflection plane. Given a single RGB image, the idea is to represent symmetry as a pixel-wise vector pointing from the current visible 2D pixel point to its symmetric point in 2D image. We call these vectors as symmetry correspondences. Each symmetry correspondence $l_i$ of pixel $p_i$ is the projection of a vector $L_i$, which is parallel to the normal vector $n_s$ of reflection plane starting from the point $P_i$ and pointing to the symmetry point $P_i'$ in 3D object frame. Therefore we designed a network to predict the symmetry correspondence. By leveraging such symmetry correspondence, we can recover both the reflection plane and further refine object pose.\\

Our network is desigend as: TBD. 

We then use initial pose $T$ predicted in keypoint prediction module and symmetry correspondence $l_i,i=1...n$ to vote for the normal vector of reflection plane. As assumed earlier, there is one symmetry plane of object, say $x-y$ plane, $y-z$ plane, or $z-x$ plane, therefore the potential normal vector of reflection plane is $(0,0,1)$, $(1,0,0)$, and $(0,1,0)$. We reproject three potential normal vectors onto the image plane under pose $T$ and calculate the cross product between each normal vector and $n$ symmetry correspondences. Since the symmetry correspondences are parallel to normal vectors in 3D space, the correct normal vector should have minimum sum of cross product expressed as follows:
\begin{equation}
    n_s = \mathrm{argmin}\sum_i\pi(n_{sj},K,T)\times l_i
\end{equation}
where $n_{js}, j = 1,2,3$ is potential normal vector, $\pi$ denotes the projection from object frame to image plane, $K$ is camera intrinsic matrix.

\subsection{Pose refinement module}
We define the pose refinement module as $\Delta T_{k+1}=h_{\theta}(e_{k}(p_i,T_k,P_i),e_{k}(l_i,T_k))$ where $\theta$ are network parameters, $k$ denotes $k$ th iteration. The input of this network is pose $T_k$, prior information of 3D coordinates of keypoints $P_i$, keypoint reprojection error $e_k(p_i,T_k,P_i)$ and symmetry reprojection error$e_k(l_i,T_k)$. The output of this network is updated pose $\Delta T_{k+1}=\varepsilon_{k+1}\in \mathbb{R}^{6}$ and thus the updated pose is $T_{k+1} = \mathrm{exp}(\varepsilon_{k+1}^{\wedge})T_k$.

The keypoint reprojection error has form of:
\begin{equation}
    e_k(p_i,T_k,P_i) =\| p_i - \pi(T_kP_i)\|^2
\end{equation}
and symmetry reprojection error is:
\begin{equation}
    e_k(l_i,T_k) =l_i^{\mathrm{T}}\pi(R_kn_{s})
\end{equation}
where $R_k$ is the rotation matrix, $n_s$ is the voted normal vector of symmetry plane mentioned in last the subsession.

We define the loss function as: 
\begin{equation}
    \mathrm{min} \|T^{-1}T_{kmax}-I_{4\times 4} \|_{\mathcal{F}}^2
\end{equation}

Essentially, we want to build a recurrent network $h_{\theta}$ to regress the pose update based on geometric errors formed by keypoint measurement $p_i$ and symmetry measurement $l_i$ by minimizing the difference of ground truth pose and estimated pose. We can do directly optimization in form of weighted least square using Levenberg-Marquardt algorithm, however the reason of using a neural network to learn pose update are twofold: it is nontrivial to design weight for two different types of measurements $p_i$ and $l_i$ to achieve a promising pose result, the measurement $p_i$ and $l_i$ may be noisy which is unable to provide with proper direction of gradient. 

The network is a fully connected network with input size $2N$, where $N$ is the number of keypoints, since we have $N$ keypoint reprojection errors and $N$ symmetry reprojection errors, and the output size is 6.\\

TODO: derive derivative for backpropogation..\\

Note: given a trained refinement network, we may evaluate the effect of conversion network by comparing the pose update of each iteration (with and without conversion network), based on the fact that when the keypoints is accurate, the initial pose would be much more accurate, resulting in smaller pose update $\Delta T_k$. 
\subsection{Conversion module}
TBD





\begin{comment}
\subsection{Proposed symmetry representation}
First assume the object has one reflection plane and we don't know which plane is. We want to train a network  representing symmetry correspondence to estimate the reflection plane, and then use both reflection plane and symmetry correspondence to estimate pose. The whole pipeline uses PVNet as baseline.

Given a single RGB image, the main idea is to represent symmetry as a pixel-wise vector pointing from the current visible 2D pixel point to its symmetric point in 2D image. (Here, we don't care whether the corresponding symmetric point is visible or not.) We call these vectors as symmetry correspondences. Basically, each symmetry correspondence $l_i$ of pixel $p_i$ is the projection of a vector $L_i$, which is parallel to the normal vector $n_s$ of reflection plane starting from the point $P_i$ and pointing to the symmetry point $P_i'$ in 3D object frame. 

The vector $L_i$ is projected by object pose $T$ onto the image plane as $l_i$, which contains, kind of, rich geometric information: first, when the length of symmetry correspondence of a certain pixel point is zero, such pixel point should pass through reflection plane in 3D space; second symmetry correspondence implicit represents more keypoints and even lines. Therefore by leveraging such symmetry correspondence, we can recover both the reflection plane and pose.

\subsection{Proposed pose estimation pipeline}
We can first use PVNet to extract keypoints $p_i, i=1...8$(maybe), its corresponding 3D object points $P_i$ and calculate initial object pose $T$. Then we train a network to predict dense symmetry correspondence $L_i,i=1...n$ where $n$ is the number of pixels within object mask. 

Then we can use pose $T$ and symmetry correspondence $L_i,i=1...n$ to recover reflection plane by voting for its normal vector. As assumed at beginning of this session, there is one symmetry plane of object, say $x-y$ plane, $y-z$ plane, or $z-x$ plane, therefore the potential normal vector of reflection plane is $(0,0,1)$, $(1,0,0)$, and $(0,1,0)$. Given the object pose $T$ and camera intrinsic matrix $K$, we can reproject three potential normal vectors onto image plane, and calculate the cross product between each normal vector and $n$ symmetry correspondences. Since the symmetry correspondences are parallel to normal vectors in 3D space, the correct vector normal should have minimum sum of cross products expressed as follows:
\begin{equation}
    \mathrm{min}\sum_i\pi(n_{sj},K,T)\times l_i
\end{equation}
where $n_{js}, j = 1,2,3$ is potential normal vector, $\pi$ denotes the projection from object frame to image plane.

Given normal vector of reflection plane $n_s$, keypoints $p_i$ extract from PVNet and its corresponding 3D point $P_i$ in object frame and symmetry correspondence $l_i$ we can easily calculate symmetry point $P_i'$ in 3D. Then we can calculate the vector $L_i$ for each keypoint $i$ and form an objective function to refine pose $P$ based on the fact that each symmetry correspondence $l_i$ is the projection of $L_i$ under pose $T$:
\begin{equation}
    \mathop {\min }\limits_{T}f(\sum_ili-\pi(T,n_s,P_i,K))
\end{equation}
Here the objective function is to minimize reprojection error between 3D vectors and 2D vectors (symmmetry correspondence). Rather than reprojecting points, we reproject lines (also call vector) here, which might be more helpful because lines have more information than points. But we can also use reprojection error of points, as the information is also available now. And we can change the form $f(.)$, for example inner product, cross product or something to make it more easy to calculate and more reasonable.

\subsection{Advantages and disadvantages}
\textbf{Disadvantage}: Not sure how hard it is to train such a network to represent vector-field feature, symmetry correspondence. Still looking at papers..

\textbf{Advantages}: this representation can implicitly represent keypoints(whatever is visible or not), lines information which can be directly used to infer symmetry and do pose estimation. We may also able to find more geometric relation between other features, such as keypoint and form our conversion network. 

\textbf{Dataset}: given 3D object model, it should be ok to generate such symmetry correspondence and project them into 2D image space. Still finding datasets to check if they have 3D model for real images. LineMOD, YCB related would be a good choice...   
\end{comment}

\subsection{Approximate EPnP as network}
This section we want to approximate EPnP\cite{lepetit2009epnp} as a network, so that we can make the whole pipeline end-to-end trainable. 
\subsubsection{Review of EPnP algorithm}
The input of EPnP algorithm are 3D-2D point correspondences in object frame and image plane, $P_i$ (homogeneous coordinates), $p_i=(u_i,v_i)$. The algorithm parameterizes $P_i$ as four control points $C_j$ as :
\begin{equation}
    P_i = \sum^{4}_{j=1}\alpha_{ij}C_j
\end{equation}
where $\sum^{4}_{j=1}\alpha_{ij} = 1$ are homogeneous barycentric coordinates, which is unique and is easy to be calculated. 

Given pose $T = \left[\begin{matrix}
R & t\\
0^{\mathrm{T}} & 1
\end{matrix} \right]$, the point $P_i$ in camera frame is expressed as $P_{ci} = TP_i$. Similarly, the control points in camera frame can be expressed as $C_{cj} = TC_j$, and we have:
\begin{equation}
    P_{ci} = \sum^{4}_{j=1}\alpha_{ij}C_{cj}
\end{equation}

Theorically when we know 4 pairs of control point in both camera frame and object frame, $C_{cj}$ and $C_{j}$, it is easily to calculate pose $T$:
\begin{equation}
    T = C_cC^{\mathrm{T}}(CC^{\mathrm{T}})^{-1}
    \label{Eq: pose_pnp}
\end{equation}
where $C_c=[C_{c1},C_{c2},C_{c3},C_{c4}]$ and $C = [C1,C2,C3,C4]$. Therefore pose estimation problem is reduced to estimate 4 control points in camera frame $C_{cj}$

Given camera pinhole model and intrinsic parameters, such as focal length $f_u, f_v$, and optical center $c_u,c_v$, we can get:
\begin{equation}
    \begin{aligned}
    \sum^{4}_{j=1}\alpha_{ij}f_ux_{cj} + \alpha_{ij}(u_c-u_i)z_{cj} =& 0\\
    \sum^{4}_{j=1}\alpha_{ij}f_vx_{cj} + \alpha_{ij}(v_c-v_i)z_{cj} =& 0\\
    \end{aligned}
\end{equation}
where $C_{cj} = [x_{cj},y_{cj},z_{cj} ]^{\mathrm{T}}$. Since the only unknown variable is $[x_{cj},y_{cj},z_{cj} ]$, it is easy to concatenate four points together as $x$ and reform the above equation as:
\begin{equation}
    M_{12\times 12}x_{12\times 1} = 0
\end{equation}
The solution $x$ lies in the null space of $M$, which can be calculated as:
\begin{equation}
    x = \sum^{N}_{k=1} \beta_kv_k
    \label{Eq: C_c solution}
\end{equation}
where $v_k$ is the null eigenvectors of matrix $M^{\mathrm{T}}M$. 

As mentioned in \cite{lepetit2009epnp}, the number of $N$, ranging from 1 to 4, depends on image noise, focal length etc. The paper discussed the solution for $\beta_k$ in 4 cases respectively and proposes to choose a proper $N$ and $\beta_k$ which yields the smallest summation of reprojection error of $P_i$ and $p_i$ pairs. The paper also proposed to use Gauss-Newton to refine the value of $\beta_k$. However, in our work, we propose to approximate the EPnP by estimating the $\beta_k$ using a neural network, called PnPNet.
\subsubsection{PnPNet}
PnPNet takes 2D keypoint $p_i$ and corresponding 3D object homogenorous coordinates $P_i$ and outputs object pose $T$. The architecture is shown in Fig \ref{fig:pnp}:
\begin{figure}[ht]
	\centering
	\includegraphics[width=1\linewidth]{files/pnp.png}
	\caption{PnPNet}
	\label{fig:pnp}
\end{figure}

The network is designed to learn the proper $\beta_k$ in Equation \ref{Eq: C_c solution}, and then the pose is calculated by Equation \ref{Eq: pose_pnp}. It first takes in homogeneous coordinates $P_i$ to calculate the four control points $C_i$. Simultaneously, it takes in detected keypoints $p_i=(u_i,v_i)$ to form $M$, and calculates the first four eigenvectors of $M^{\mathrm{T}}M$, namely $v_k$. Good $\beta_k$ should maintain the distance between four control points in 3D space, thus the following equation should hold for each $i,j$ ranging from 1 to 4:
\begin{equation}
    \|\sum_{k=1}^4 \beta_kv_k^{[i]}-\sum_{k=1}^4 \beta_kv_k^{[j]}\|^2=\|C_i-C_j\|^2
\end{equation}
where $v_k^{[i]}$ is $i$th sub-vector of vector $v_k$ that corresponds to control point $C_{ci}$. Therefore we set six point distances of both control points and sub-vector as network input and use a simple three layer perceptron to predict a proper $\beta_k$ for each vector $v_k$. Since EPnP algorithm will generate a pose based on 3D-2D correspondence, we design the following loss to enforce the PnPNet to generate a good pose:
\begin{equation}
    L1 = \|\sum_{k=1}^4 \beta_kv_kC(CC^{T})^{-1}T_{gt}^{-1}-I_{4\times 4}\|_{\mathcal{F}}^2
\end{equation}
where $T_{gt}$ is the pose groundtruth. 

(Note: This network can be trained separately, and we can generate the training data in simulation using Gaussian noised image points and clean 3D object point. As for pose label, we can generate it by EPnP algorithm or directly use ground truth pose in simulation.)

There is another loss L2, which seems to be more reasonable? Please refer to \cite{lepetit2009epnp}'s equation 10.
\begin{equation}
    L2 =  \|\sum_{k=1}^4 \beta_kv_k^{[i]}-\sum_{k=1}^4 \beta_kv_k^{[j]}\|^2 - \|C_i-C_j\|^2
\end{equation}
But this loss doesn't have pose supervision...


\section{Using Symmetry as Geometry Constraint}
{
\renewcommand{\vec}[1]{\boldsymbol{#1}} % Uncomment for BOLD vectors.
\subsection{Symmetry in 3D Geometry (there may be errors)}
Suppose we have predicted symmetric correspondences of an object in the RGB image, i.e. for every pixel $p$, its symmetric correspondence in the image is $p'$. For each $p$ and $p'$ pairs, the corresponding 3D coordinates expressed in object frame are $P$ and $P'$. As indicated in FIGURE.. We define the normal of symmetric plane $\vec{n}$ in camera frame is $\vec{n_c}$, the distance between the camera origin and the plane is $d$. The intrinsic matrix of the camera is $K$.

Given a certain point $P_s$ in symmetry plane and the normal $\vec{n}$ in object frame , we have:
\begin{equation}
    P' = P + 2\Vec{n}\vec{n}^{T}(P_s - P)
    \label{eq: symmetry}
\end{equation}
Suppose object pose is $\left[R|t\right]$, then we have $P_c = RP + t$ and $\vec{n_c} = R\vec{n}$, the equation \ref{eq: symmetry} can be reformed as:
\begin{equation}
\begin{aligned}
    RP' &= RP + 2R\Vec{n}\vec{n}^{T}R^{T}(RP_s - RP)\\
    P'_c &= P_c + 2\Vec{n_c}\vec{n_c}^{T}(P_{sc} - P_c)
    \label{eq: symmetry2}
\end{aligned}
\end{equation}
Then $d = -P_{sc}^{T}\vec{n_c}$. When we choose $P_s$ as center of object, $P_{sc}$ is translation vector $t$, $d$ is projection of $P_{sc}$ on $\vec{n_c}$, which explains symmetry plane can just recover the 5 degrees of freedom. 
Rearrange equation \ref{eq: symmetry2}, we have:
\begin{align}
P_c' = \left[
\begin{matrix}
I_3-2\vec{n_c}\vec{n_c}^T & -2d\vec{n_c} \\
\vec{0} & 1
\end{matrix}\right] P_c \label{equ:symmetry_transform}
\end{align}

Denote:
\begin{align}
R_s &= I_3-2\vec{n_c}\vec{n_c}^T, \label{equ:R_s}\\
t_s &= -2d\vec{n_c},\label{equ:t_s}
\end{align}

then:$P_c' = R_s P_c + t_s$.

According to the pinhole camera model, we know that
\begin{align}
s\Tilde{p} &= KP_c \\
s'\Tilde{p}'&=K\left(R_sP_c+t_s\right)
\end{align}
where $\Tilde{p}$ is the homogeneous coordinates of $p$. Define $x = K^{-1}\Tilde{p}$, $x' = K^{-1}\Tilde{p}'$, we can get:
\begin{align}
x'^Tt_s^\wedge R_sx=0 \label{equ:geometry_constraint}
\end{align}
which is the same as two-view epipolar geometry. Therefore, at least 5 paris of symmetric correspondences are needed to calculate $R_s$ and $t_s$ (i.e. $\vec{n_c}$ and $d$). We can also use the classic eight-point-algorithm to calculate symmetric plane.

It should be noted that there are geometry constraints between the 

The geometric constraints between symmetric plane and pose $\left[R|t\right]$ and $R_s$ and $t_s$ are (double check the third one):
\begin{equation}
\begin{aligned}
t_s &= 2t^{\mathrm{T}}R\vec{n}R\vec{n}\\
R_s &= I - 2R\vec{n}R\vec{n}^{\mathrm{T}}\\
t_s^\wedge R_s &= 2t^{\mathrm{T}}R\vec{n}(R\vec{n})^\wedge 
\end{aligned}
\end{equation}
%\begin{figure}
%	\centering
% 	\includegraphics[width=0.6\linewidth]{./files/symmetric_plane.png}
%	\caption{symmetric plane}
%	\label{fig:symmetric_plane}
%\end{figure}

\subsection{Pipeline}
% idea1: pipeline: use epipolar geometry constraint to explicitly calculate symmetric plane.
\begin{figure}
	\centering
	\includegraphics[width=1\linewidth]{./files/pipeline1.png}
	\caption{pipeline1}
	\label{fig:pipeline1}
\end{figure}
% problems:
% the solving of $x'^{T}t_{s}^{\wedge}R_{s}x=0$ need to be differentiable.

\begin{figure*}
	\centering
	\includegraphics[width=1\linewidth]{./files/pipeline2_update.png}
	\caption{pipeline2}
	\label{fig:pipeline2}
\end{figure*}

\subsubsection{pipeline2}
There are three kinds of representations of symmetry: sparse symmetric correspondences, dense symmetric correspondences and symmetric plane. They all encodes the symmetry information.

We first use PVNet structure to predict sparse symmetric correspondences (2D keypoints). They could be later incorporated with their corresponding 3D points in order to solve the PnP problem, which estimates the relative pose $\left[R|t\right]$.

We also use another network to predict dense symmetric correspondences $p_d$ and $p_d'$, i.e. for every $p_d$ of the object in 2D image, the network predicts the vector pointing from $p_d$ to $p_d'$. Note that the symmetric plane can be represented by the normal $\vec{n}$ and the distance $d$. We then design a new network that takes symmetric correspondences $p_d$ and $p_d'$ as inputs and predicts the dense representation of symmetric plane. To be specific, every pair of correspondence produces a symmetric plane $\vec{n}_{i}$ and $d_i$, as well as its probability $c_{i}$. By voting, we can get the final symmetric plane $\vec{n}$ and $d$ with the highest probability. With equation \ref{equ:R_s} and \ref{equ:t_s}, we can directly obtain $R_s$ and $t_s$ from $\vec{n}$ and $d$.

Since $x_d$ and $x_d'$ are symmetric correspondences, they should satisfy the geometry constraint illustrated by equation \ref{equ:geometry_constraint}. However, the estimation of both symmetric correspondences and symmetric plane are not precise, so $x_d'^{T}t_{s}^{\wedge} R_{s}x_d$ is not equal to 0. Therefore, we can use $x_d'^{T}t_{s}^{\wedge} R_{s}x_d$ as a part of the loss function.
\begin{align}
l_{symmetry, dense} = \sum_i\left|x_{d,i}'^{T}t_{s}^{\wedge} R_{s}x_{d,i}\right|
\end{align}

This is also the same for sparse symmetric correspondences
\begin{align}
l_{symmetry, sparse} = \sum_i\left|x_{s,i}'^{T}t_{s}^{\wedge} R_{s}x_{s,i}\right|
\end{align}

Another geometry constraint comes from the relationship between $\left[R_s|t_s\right]$ and $\left[R|t\right]$, i.e. 
\begin{align}
R_s&=I-2\vec{n}\vec{n}^{T} \\
ts&=\pm2\vec{n}\vec{n}^{T}t \\
\vec{n}&=R^{T}\vec{n}_{0}
\end{align}
where $\vec{n_0}$ is the normal of the symmetric plane in the object coordinate. (Note that there are some bugs in equation \ref{equ:symmetry_transform}, $d$ and $\vec{n}$ need to be defined well, or else it may be $2d\vec{n}$ instead of $-2d\vec{n}$). A loss can be designed according to this constraint.
% idea2: voting: use network to generate symmetric plane for every correspondence pairs (and vote), which satisfies the epipolar constraint and other geometry constraint. For example, every $x$ & $x'$ produce a $\left(\vec{n}, d\right)$ and $c_{i}$ (probability), then every corresponding pair votes a symmetric plane.


\subsection{unsupervised learning pose estimation without keypoint detection}

Based on equation \ref{equ:geometry_constraint} and definition of $x$, we have:
\begin{equation}
    (RP'+t)^{\mathrm{T}}t_s^\wedge R_s(RP+t)=0
    \label{Eq: sym_pose}
\end{equation}
this equation shows the relationship between pose and symmetry information which can be used as loss for unsupervised learning. Therefore we can build the following pipeline to estimate the object pose end-to-end.
\begin{figure*}
	\centering
	\includegraphics[width=1\linewidth]{./files/2.png}
	\caption{unsupervised}
	\label{fig:unsupervised}
\end{figure*}
}


==> Backup/05_experimental_results.tex <==
\section{Experimental Evaluation}
\label{Section:Experimental:Evaluation}

\subsection{Experimental Setup}
\label{Subsection:Experimental:Setup}

\subsection{Analysis of Results}
\label{Subsection:Analysis:of:Results}

\subsection{Ablation Study}
\label{Subsection:Ablation:Study}

==> Backup/05_pose_regression_old.tex <==
\subsection{Pose Regression}
\label{Subsection:Pose:Regression}

The second module of HybridPose outputs a 6D object pose $R_I\in SO(3), \bs{t}_I\in \R^3$ for the input image $I$. To make the notations uncluttered, denote the predicted keypoints, edge vectors, and symmetry correspondences as $\bs{p}_k^{2D}\in \R^2, 1\leq k \leq |\set{K}|$, $(\bs{v}_{e}^{2D}\in \R^2), 1\leq e \leq |\set{E}|$, and  $(\bs{q}_{s,1}^{2D}\in \R^2,\bs{q}_{s,2}^{2D}\in \R^2), 1\leq s \leq |\set{S}|$, respectively. Our formulation also uses the homogeneous coordinates $\bs{q}_{s,1}\in \R^3$ and $\bs{q}_{s,2}\in \R^3$ of $\bs{q}_{s,1}^{2D}$ and $\bs{q}_{s,2}^{2D}$, respectively. Consider a 3D keypoint template, whose 3D keypoint coordinates in the canonical coordinate system $\Sigma$ are $\bs{p}_k^{3D}, 1\leq k \leq |\set{K}|$. Denote $\set{P}_{R,\bs{t}}:\R^3\rightarrow \R^2$ as the perspective projection. HybridPose generalizes PnP fitting~\cite{Lepetit:2009:EAO,Persson_2018_ECCV}, which involves the following constraints: $\forall k, e, s,$
\begin{align}
\bs{0} & \approx \bs{r}^{\set{K}}_{R,\bs{t}}(\bs{p}_k^{2D}):= \set{P}_{R,\bs{t}}(\bs{p}_k^{3D}) - \bs{p}_k^{2D}\approx \bs{0}, \label{Eq:1} \\    
\bs{0} & \approx \bs{r}^{\set{E}}_{R,\bs{t}}(\bs{v}_e^{2D}):=\set{P}_{R,\bs{t}}(\bs{p}_{e_t}^{3D})-\set{P}_{R,\bs{t}}(\bs{p}_{e_s}^{3D}) - \bs{v}_e^{2D}, \label{Eq:2} \\
0 &\approx r^{\set{S}}_{R,\bs{t}}(\bs{q}_{s,1}^{2D},\bs{q}_{s,2}^{2D}):= (\bs{q}_{s,1}\times \bs{q}_{s,2})^T R\bs{n}_{r}^{3D}.\label{Eq:3}
\end{align}
where $e_s$ and $e_t$ are end vertices of edge $e$, and $\bs{n}_r^{3D}\in \R^3$ is the normal of the reflection symmetry plane in the canonical system. In other words, (\ref{Eq:1}) and (\ref{Eq:2}) measures the projection error for key points and edge vectors, respectively. (\ref{Eq:3}) is the epipolar constraint for symmetric correspondences~\cite{Ma:2003:IVI}. 

To model outliers in the predictions, we associate each predicted element with a weight, i.e., $w_{\set{K},k}\in [0,1],1 \leq k \leq |\set{K}|$, $w_{\set{E},e} \in [0,1], 1\leq e \leq |\set{E}|$, and $w_{\set{S},s} \in [0,1], 1\leq s \leq n_{I}$ for keypoints, edge vectors, and symmetry correspondences, respectively. This pose regression module alternates between pose regression with fixed weights and updating weights. The weight updating module employs a neural network with trainable weights $\alpha$. The initial weights are given by $w_{\set{K},k} = 1/\sigma^2_{\keypoint}$, $w_{\set{E},e} = 1/\sigma^2_{\edgevec}$, and $w_{\set{S},s} = 1/\sigma^2_{\symmetry}$ where
\begin{align}
\sigma^2_{\keypoint} & = E[\|\bs{r}^{|\set{K}|}_{R^{\star},\bs{t}^{\star}}(\bs{p}_{k}^{2D})\|^2] ,\ \  \sigma^2_{\edgevec}  = E[\|\bs{r}^{\set{E}}_{R^{\star},\bs{t}^{\star}}(\bs{v}_e^{2D})\|^2] \nonumber \\
\sigma^2_{\symmetry} & =E[\big(r^{\set{S}}_{R^{\star},\bs{t}^{\star}}(\bs{q}_{s,1}^{2D},\bs{q}_{s,2}^{2D})\big)^2] 
\label{Eq:Sigma:Defn}
\end{align}
where the expectation is taken among the validation set in the 10-fold valuation setting with-respect to pre-trained prediction networks and ground-truth object poses  

\noindent\textbf{Regression sub-module.} HybridPose solves the following non-linear least squares to obtain the optimized object pose at the each iteration:
\begin{align}
\min\limits_{R, \bs{t}} & \ \sum\limits_{k}w_{\set{K},k} \|\bs{r}^{|\set{K}|}_{R,\bs{t}}(\bs{p}_{k}^{2D})+  \sum\limits_{e}w_{\set{E},e} \|\bs{r}^{\set{E}}_{R,\bs{t}}(\bs{v}_e^{2D})\|^2 \nonumber \\
+ &  \sum\limits_{s=1} w_{\set{S},s} \big(r^{\set{S}}_{R,\bs{t}}(\bs{q}_{s,1}^{2D},\bs{q}_{s,2}^{2D})\big)^2
\label{Eq:Pose:Regression:Obj}
\end{align}
HybridPose employs the Gauss-Newton method for numerical optimization. The initial solution at the each iteration is given by the optimal solution at the previous iteration. To obtain the initial solution at the first iteration, HybridPose generalizes the approach of first solving the affine object pose and then projecting the resulting affine object pose onto the space of rigid motion~\cite{Ma:2003:IVI}. The difference lies in extending the objective function to incorporate constraints of key points, edge vectors, and symmetry correspondences. Please refer to the supplemental material for details. 

Training the pose regression module requires computing the gradient of the optimal solution to (\ref{Eq:Pose:Regression:Obj}) with respect to elements that define the objective function. The following proposition presents a general formulation for this purpose:
\begin{proposition}
Consider an objective function described as $f(\bs{x},\bs{y})$. Let $\bs{y}^{\star}(\bs{x})$ be the function defined implicitly as 
\begin{equation}
\bs{y}^{\star}(\bs{x}):= \min\limits_{\bs{y}}\ f(\bs{x},\bs{y}).
\end{equation}
Then the derivatives of $\bs{y}^{\star}$ with respect to $\bs{x}$ are given by 
\begin{equation}
\frac{\partial \bs{y}^{\star}}{\partial \bs{x}}(\bs{x}) = \left[\frac{\partial^2 f}{\partial^2 \bs{y}}(\bs{x}, \bs{y}^{\star})\right]^{-1}\cdot \frac{\partial^2 f}{\partial \bs{x} \partial \bs{y}}(\bs{x}, \bs{y}^{\star})
\label{Eq:Partial:Derivation}
\end{equation}
\end{proposition}
To apply (\ref{Eq:Partial:Derivation}) in our setting, we simply let $\bs{x}$ collect the predicted key points, edge vectors, symmetry correspondences, and the weights. $\bs{y}\in \R^6$ is a free parameterization of the space of rigid transformations. Note that (\ref{Eq:Partial:Derivation}) admits efficient computation, as it involves inverting a $6\times 6$ matrix.  

\noindent\textbf{Weighting sub-module.}HybridPose updates the element weights based on quantities derived from the current solution. The motivation comes from the success of using iteratively reweighted schemes for robust regression. However, a hand-crafted robust norm is blind to the input data and may lead to sub-optimal results. Recent works~\cite{Yi_2018_CVPR,DBLP:conf/eccv/RanftlK18,DBLP:conf/nips/KimLJMS18,Huang_2019_CVPR} have shown the advantages of making the weighting procedure learnable. However, these approaches mainly consider the accuracy of the input elements, they do not consider robustness of the resulting system, which is particularly important when predictions are noisy.  

To ease the discussion, let us rewrite the objective function in (\ref{Eq:Pose:Regression:Obj}) as $\sum_{i=1}^{N}w_i \|\bs{f}_i(\bs{y})\|^2$, where each term accounts for one constraint in (\ref{Eq:1})-(\ref{Eq:3}). Let $k_i$ be the correspondence type for $f_i$, e.g., $k_i = 1$ for key points, $k_i = 2$ for edge vectors, and $k_i = 3$ for symmetry correspondences. With this setup, we model the weighting sub-module as a two-layer network. The first layer admits the following form:
\begin{equation}
\overline{w}_i = \frac{\alpha_{k_i 1}^2}{\alpha_{k_i 2}^2 + \|\bs{f}_i(\bs{y}^{\star})\|^{2\alpha_{k_i 3}} + \alpha_{k_i 4}^2 \|\bs{f}_i(\bs{y}^{\star})\|^{2\alpha_{k_i 5}}} 
\label{Eq:Weighting:Scheme}
\end{equation}
where $\alpha_{k_ij}$ are hyper-parameters, and (\ref{Eq:Weighting:Scheme}) uses different hyper-parameters to model each type of terms. Note that when setting $\alpha_{k_i 1} = \alpha_{k_i 2} = \sigma$, $\alpha_{k_i 3} = 1$, and $\alpha_{k_i 4} = \alpha_{k_i 5} = 0$, then (\ref{Eq:Weighting:Scheme}) becomes $w_i = \frac{\sigma^2}{\sigma^2 + \|\bs{f}_i(\bs{y}^{\star})\|^2}$, which is the reweighting scheme for $L^0$ optimization.  

The second layer re-scales the weight $w_i = \overline{w}_i e^{z_i}$, where $z_i\in \R$ is a parameter to choose. To set $z_i$, we consider the approximated Hessian matrix of the optimization problem
$$
H: = \sum\limits_{i=1}^{N} \overline{w}_i e^{z_i} (\nabla \bs{f}_i) (\nabla\bs{f}_i)^T,
$$
where $\nabla\bs{f}_i$ is the Jacobi of $\bs{f}_i$ at the current optimal solution $\bs{y}^{\star}$. In the supplemental material, we provide an analysis which shows that the condition number $\kappa_{H} = \lambda_{\max}(H)/\lambda_{\min}(H)$ dictates the regression error under a robust setting. 
\begin{proposition}
The derivative of $\kappa_H$ with respect to $z_i$ at $z_i = 0, 1\leq i \leq N$ is given by
$$
\frac{\partial \kappa_H}{\partial z_i}:= \frac{\overline{w}_i}{\lambda_{\min}(H)}\big(\|\nabla\bs{f}_i^T\bs{u}_{\max}\|^2-\kappa_H\|\nabla\bs{f}_i^T\bs{u}_{\min}\|^2\big) 
$$
where $\bs{u}_{\min}$ and $\bs{u}_{\max}$ are the eigen-vectors that correspond to the minimum and maximum eigen-values of $H$.
\label{Prop:Kappa:Derivative}
\end{proposition}
In light of (\ref{Prop:Kappa:Derivative}), we set the output of the weighting sub-module as $w_i = \overline{w}_i e^{-\alpha_{0}\frac{\partial \kappa(H)}{\partial z_i}}$, where $\alpha_0$ is a hyper-parameter shared by the pose regression module. 
\begin{proposition}
(\textbf{Informal}) Under mild conditions, the generalized reweighting scheme described above converges to a stationary point. 
\end{proposition}






==> Backup/06_network_training_old.tex <==
\subsection{HybridPose Training}
\label{Subsection:Network:Training}

Given the network design in the preceding section, we denote HybridPose as $\set{R}(f_{\theta}^{\set{K}}(I),f_{\phi}^{\set{E}}(I),f_{\gamma}^{\set{S}}(I)), \alpha)\rightarrow (R\in SO(3),\bs{t}\in \R^3)\in \R^{3\times 4}$, which takes an input image and outputs its object pose denoted as $R$ and $\bs{t}$. We consider four loss terms for training HybridPose. The three loss terms $l_{\set{K}}(\theta)$, $l_{\set{E}}(\phi)$, and $l_{\set{S}}(\gamma)$ are used train prediction networks of key-points, edge vectors, and symmetry correspondences, respectively. Each loss employs a corresponding label dataset and a standard loss measure. Due to the space constraint, we leave the details to the supplemental material. The fourth loss term employs an imageset $\set{I}$ and the corresponding pose labels $(R_I^{\star}\in SO(3), \bs{t}_I^{\star}\in \R^3), I\in \set{I}$. Putting all loss terms together, we define the following optimization problem for training the prediction networks and the parameters $\alpha$ of the weighting module:
\begin{align}
\min\limits_{\theta,\phi,\gamma,\alpha } & \ \sum\limits_{I\in \set{I}}\|\set{R}(f_{\theta}^{\set{K}}(I),f_{\phi}^{\set{E}}(I),f_{\gamma}^{\set{S}}(I)), \alpha)-(R_{I}^{\star},\bs{t}_I^{\star})\|_{\set{F}}^2  \nonumber \\
&+\lambda_{\keypoint} l_{\keypoint}(\theta) + \lambda_{\edgevec} l_{\edgevec}(\phi) + \lambda_{\symmetry}l_{\symmetry}(\gamma) 
\label{Eq:Total:Loss}
\end{align}
where $\lambda_{\keypoint}$, $\lambda_{\edgevec}$, and $\lambda_{\symmetry}$ are tradeoff parameters, and we determine them through 10-fold cross-validation. 

We solve (\ref{Eq:Total:Loss}) in three phases. The first phase initializes each prediction network by minimizing its corresponding loss, i.e., by omitting the last term of (\ref{Eq:Total:Loss}). The second phase fixes the prediction networks and optimizes $\alpha$. The third phase fine-tunes all variables. At all phases, network training involves ADAM with back-propagation~\cite{KingmaB14}. Mote that the gradients of $\set{R}(f_{\theta}^{\set{K}}(I),f_{\phi}^{\set{E}}(I),f_{\gamma}^{\set{S}}(I)), \alpha)$ employ (\ref{Eq:Partial:Derivation}). 

